Unsupervised Feature Learning through Divergent Discriminative Feature Accumulation

Unlike unsupervised approaches such as autoencoders that learn to reconstruct their inputs, this paper introduces an alternative approach to unsupervised feature learning called divergent discriminative feature accumulation (DDFA) that instead continually accumulates features that make novel discriminations among the training set. Thus DDFA features are inherently discriminative from the start even though they are trained without knowledge of the ultimate classification problem. Interestingly, DDFA also continues to add new features indefinitely (so it does not depend on a hidden layer size), is not based on minimizing error, and is inherently divergent instead of convergent, thereby providing a unique direction of research for unsupervised feature learning. In this paper the quality of its learned features is demonstrated on the MNIST dataset, where its performance confirms that indeed DDFA is a viable technique for learning useful features.

==> nnmacros.tex <==
%% $Id: nnmacros.tex,v 1.28 2005/09/28 21:18:37 jbednar Exp $
%%
%% Standard set of LaTeX macros and declarations for the NN group
%%
%% Originally based on risto's com.tex
%%
%% Because of \usepackage{hyperref}, this file should be included
%% *after* all other packages.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Add ability to check for PDFTeX

\newif\ifpdf
\ifx\pdfoutput\undefined
  \pdffalse
\else
  \pdfoutput=1
  \pdftrue
\fi

%% Macro useful for figuring out if a TeX command has been defined
%%
\def\ifundefined#1{\expandafter\ifx\csname#1\endcsname\relax}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Packages required


% Because of this call, the "graphics" interface can't be used in
% conjunction with this file.  
%
\ifpdf\PassOptionsToPackage{pdftex}{graphicx}\fi
\usepackage{graphicx}

%% If you want to supply options to the hyperref package, you can add :
%% 
%% \PassOptionsToPackage{...}{hyperref} 
%%
%% in your source file before any \usepackage commands.  To turn
%% off hyperlinks altogether, you can use: 
%%
%% \PassOptionsToPackage{draft}{hyperref} %% Turn off hyperref links
%%
\ifpdf
%% Highlights links in PDF files
\usepackage{hyperref}
%% Highlights bibliography links
\newcommand{\biblink}[2]{\htmladdnormallink{#1}{#2}}
\fi

% From the LaTeX2HTML distribution.
\usepackage{html}%   
%
% If you don't have or want LaTeX2HTML when running this at home, just
% copy /u/nn/tex/latex2html/texinputs/html.sty to somewhere   
% in your TEXINPUTS path and ignore the rest of LaTeX2HTML.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% From risto's com.tex:

%%% Generates a \tt quotation without indentation
%\def\quotation{\list{}{\listparindent 0.0em
%    \setlength{\parindent}{0.0in}
%    \renewcommand{\baselinestretch}{1}\small\normalsize\tt
%    \renewcommand{\arraystretch}{1}
%%    \itemindent\listparindent
%    \setlength{\leftmargin}{0.0in}
%    \parsep 0pt plus 1pt}\item[]}
%\let\endquotation=\endlist

%% I like to tighten up my captions and tables
\newcommand{\mycapdefs}{\renewcommand{\baselinestretch}{1}\small}
\newcommand{\mytabdefs}{\renewcommand{\arraystretch}{1}\small}

%% Get it?
\hyphenation{Miik-ku-lai-nen}

%% I don't like pages with only figures on them
\renewcommand{\topfraction}{0.9}
\renewcommand{\floatpagefraction}{0.8}
\renewcommand{\dbltopfraction}{0.9}
\renewcommand{\dblfloatpagefraction}{0.8}
\renewcommand{\textfraction}{.15}

%% Simple PostScript picture inclusion macros using the graphicx package
%%
%% These three commands have been provided for backwards compatibility
%% only.  You should not use them in new documents, because the 
%% non-standard argument format causes trouble with packages that expect
%% LaTeX-style  arguments, such as AucTeX, emacs font-lock, and
%% LaTeX2HTML.  Instead use the \pspic or \pdfpic macros (below).
%%
\begin{latexonly}
\def\putpicture   #1 (#2)\centerline{\includegraphics[totalheight=#2]ps/#1.ps}
\def\hputpicture  #1 (#2){\centerline{\includegraphics[width=#2]{ps/#1.ps}}}
\def\hvputpicture #1 (#2 by #3){\centerline{\includegraphics[width=#2,totalheight=#3]{ps/#1.ps}}}
\end{latexonly}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% \scribbledraft: Provides a single-column mode with lots of space
%% to write comments on, e.g. for giving to a coauthor.
%%
%% To use, add \scribbledraft before \begin{document} but after
%% all your \usepackage commands.
%%
%% Tips:
%%
%% If the formatting doesn't look right, you may have to comment out
%% your document style (e.g. \usepackage{<confname>}) and instead use
%% \usepackage{nntwocolumn}.  Usually it will only be the first 
%% page that has problems, though; that's where style files usually
%% mess with the page widths and lengths.
%%
%% If you get lines sticking past the edge of the column, try adding
%% \sloppy just after \scribbledraft.
%%
%% If your document has figure or figure* environments that come out much
%% too small in \scribbledraft mode, you may be able to fix them by
%% changing them to fullfigure or fullfigure* environments, which are
%% defined below.  However, you may find that the result is no longer
%% centered properly or is the wrong width.  If so, you might need to add
%% a \setlength\originalwidth{6.5in} or \setlength\marginoffset{0in}
%% after \scribbledraft, adjusting those two values to fix the width and
%% left margin.  
%%
\newcommand{\scribbledraft}{
  \newlength\marginoffset\setlength\marginoffset{-0.5in}
  \newlength\nominalwidth\setlength\nominalwidth{3.5in}
  \newlength\nominalmargin\setlength\nominalmargin{0.5in}
  \setlength\topmargin{0.5in}
%% \setlength\oddsidemargin{0.5in}
%% \setlength\evensidemargin{0.5in}
\setlength\oddsidemargin{\nominalmargin}
\setlength\evensidemargin{\nominalmargin}
\setlength\textheight{8in}
\setlength\textwidth{\nominalwidth}
\setlength\footskip{20pt}
\setlength\marginparwidth{2.5in}
\pagestyle{plain}
\onecolumn
% Some styles (e.g. cogsci, nntwocolumn) call \twocolumn in \maketitle,
% so here we define it as a no-op
\renewcommand{\twocolumn}[1][]{##1\bigskip\bigskip} 
%%
\renewcommand{\forcedoublecolumnfigurestart}
{\setlength\textwidth{\originalwidth}%
\hspace*{\marginoffset}%
\begin{minipage}{\originalwidth}}
%%
\renewcommand{\forcedoublecolumnfigureend}
{\end{minipage}\setlength\textwidth{\nominalwidth}}
}
%% Save original value here for later
\newlength{\originalwidth}\setlength{\originalwidth}{\textwidth}
%%
\newcommand{\forcedoublecolumnfigurestart}{}
\newcommand{\forcedoublecolumnfigureend}{}
%%
\newenvironment{fullfigure}[1][tbp]
{\begin{figure}[#1]\forcedoublecolumnfigurestart}
{\forcedoublecolumnfigureend\end{figure}}
%%
\newenvironment{fullfigure*}[1][tbp]
{\begin{figure*}[#1]\forcedoublecolumnfigurestart}
{\forcedoublecolumnfigureend\end{figure*}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Conditional picture inclusion macros using the graphicx package
%%
%% If you use \pdfpic (below) when specifying a picture, you
%% can use \psdraftlevel (also below) to specify which ones to include
%% for a printout (e.g. to save print time or file size, or to print
%% color pages separately).  It's also handy to have the type of picture
%% declared in the source file this way, as a clue to what type of
%% picture is involved.  Just ignore this if it is not needed.

%% First, declare some symbolic constants representing the different
%% classes of images.  These definitions shouldn't ever need changing, 
%% but new ones can be added in between if needed.
%%  
\def\psnone{100}        % No picture should be included
\def\psline{80}         % Black and white line drawings only
\def\psmono{60}         % Monochrome images only
\def\pscolororbw{40}    % Images for which color is optional
\def\pscolor{20}        % Images for which color is required
\def\psall{0}           % All pictures should be included


%% The \psdraftlevel command determines which pictures should actually
%% be included, while other pictures merely have their bounding
%% box drawn in to save time or file size, or to print on printers
%% with insufficient memory.  It is optional, but if used, should
%% presumably be in the preamble. Each of the above levels is
%% inclusive of the preceding ones (those with lower numbers), so
%% \mono includes line drawings too, and \color includes line, mono,
%% and color pictures. 
%%
%% Example:  To include all pictures (the default),
%%   \psdrafttype{\psall}
%%
%% Example:  To include all pictures which make sense in monochrome,
%%   \psdrafttype{\pscolororbw}
%%
%% Example:  To include only line drawings, i.e. pictures likely to be
%% very small in file size, 
%%   \psdrafttype{\psline}
%%
%% Below, 0 is hardcoded instead of \psall because of problems 
%% with some versions of latex2html
\newcount\psdraftlevel \psdraftlevel=0
\newcommand{\psdrafttype}[1]{\psdraftlevel=#1}


%% Including PDF, JPG, PNG, or TIF pictures in PDFLaTeX documents,
%% (as well as EPS pictures in LaTeX documents)
%%
%% \pdfpic[category]{width}{height}{[dir/]filename}{filetype}
%%
%%
%% Arguments:
%%
%% The "category" argument is optional; if present it should indicate the
%% type of image the file represents, i.e. \psline for a line drawing,
%% \pscolor for a color photo, \pscolororbw for an image that is readable
%% either in color or monochrome, \psnone for a blank space, etc.  For 
%% a given run, the actual image is included only if the the
%% \psdrafttype is low enough.  For example, if \psdrafttype}{\psmono}
%% has been specified, all line and monochrome pictures are included,
%% but color pictures will be represented only by a bounding box.  If
%% "category" is omitted then the image will always be displayed,
%% regardless of draftlevel.
%%
%% Either or both of the length arguments "length" and "width" can be 
%% omitted if they are replaced by "!", which indicates that that
%% dimension should scale proportionally.  (If both are "!", then the
%% image is left at the natural size of the image, whatever that might
%% be for a given filetype.)  A dummy image (type \psnone) must have
%% both "length" and "width" specified, since they cannot be read from
%% a file.
%%
%% The argument "[dir/]filename" should be the complete path to your
%% picture file, minus the final extension, which in turn goes in the 
%% {filetype} argument.  For instance, to access "./images/pretty.jpg",
%% use \pdfpic{!}{!}{images/pretty}{jpg}.  
%%
%% 
%% Tips and examples:
%% 
%% Filetypes (i.e., extensions) of jpg, png, pdf and tif are currently
%% supported. Of these you should usually use pdf for line drawings,
%% jpg for photographs, and tif or png for non-photograph bitmap images.
%% 
%% Usually, it is best to specify that a picture be fixed in size
%% horizontally if it extends across the page, so that it still fits
%% on the page properly if the margins, number of columns, etc. are
%% changed.  
%%
%% Example: To insert a monochrome PNG picture images/sample.png, scaled
%% to be as wide as the current page,        
%%   \pdfpic[\psmono]{\textwidth}{!}{images/sample}{png}
%%
%% Example: To insert a line drawing images/sample.pdf, scaled to be as
%% half as wide as the page, rotated 90 degrees counterclockwise, and
%% framed with a thin, snug outline,
%%   \frame{\rotatebox{90}{\pdfpic[\psline]{!}{0.5\textwidth}{images/sample.pdf}{pdf}}}
%%
%% Example: To insert a dummy 3" x 2" space for pasting in a picture 
%% later, when no image file actually exists on disk,
%%   \pdfpic[\psnone]{3in}{2in}{Paste feller:science96 figure 3 here}{}
%%
%% If this command is used under LaTeX, the filetype is ignored and 
%% one of type eps and ending in .ps is assumed.  If you do use such EPS 
%% files, make sure that they are truly EPS (i.e., have a bounding box)
%% and not just PostScript.
%%
%%
\newcommand{\pdfpic}[5][\psall]{\includepdfpic[#1]{#2}{#3}{#4}{#5}{}}%


%% Same as \pdfpic but clips to boundary of box
\newcommand{\pdfpicclip}[5][\psall]{\includepdfpic[#1]{#2}{#3}{#4}{#5}{clip=True,}}%



%% Old-style interface for inserting PostScript pictures into LaTeX
%% documents:
%%
%%
%% This interface only supports PDF and EPS filetypes, and is included
%% for backwards compatibility with older documents developed in LaTeX.
%% Such documents can be converted to work with PDFLaTeX simply by
%% converting all of the EPS files they include to PDF.  For instance,
%% (in csh):
%%
%% foreach psfile (ps/*.ps) 
%%   epstopdf "${psfile}"
%% end
%%
%% That way PDFLaTeX will find the ps/*.pdf files, and LaTeX will find
%% the ps/*.ps files.  Be sure to check the generated .pdf figures
%% carefully; sometimes the translation process generates visible
%% artifacts.  For instance, sometimes you can see fringes around
%% sharp, high-contrast borders in images, like those when converting
%% bitmaps to JPEG.
%%
%% 
%% This macro is used just like \pdfpic, except that you should omit the
%% filetype (because only one filetype is supported for each platform)
%% and the directory (which is assumed to be ./ps/):
%%
%% \pspic[category]{width}{height}{filename}
%%
\newcommand{\pspic}[4][\psall]{\pdfpic[#1]{#2}{#3}{ps/#4}{pdf}}
\newcommand{\pspicclip}[4][\psall]{\pdfpicclip[#1]{#2}{#3}{ps/#4}{pdf}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% Implementation for \pdfpic, etc.; shouldn't usually 
%% be called directly.  Arguments are same as for \pdfpic
%% except that a 6th argument is accepted, and passed
%% directly to \includegraphics
%%
\newcommand{\includepdfpic}[6][\psall]{%
\def\pdfpicFileType{#5}%
\def\pdfpicFileExt{#5}%
%%
%% Assume .ps under LaTeX
\ifpdf\else% 
\def\pdfpicFileType{eps}%
\def\pdfpicFileExt{ps}%
\fi%
%%
%% Dummy picture: empty box (not even a frame).
%% Unspecified heights default to \unitlength
\ifx#1\psnone%
\resizebox{#2}{#3}{\begin{picture}(1,1)\end{picture}}%
%%
%% Draft picture: framed box with filename inside.
%% This looks fine with dvips, but it confuses xdvi
%% for some reason, which draws an extra box with the
%% natural size of the image. 
\else{\ifnum#1<\psdraftlevel%
\frame{\resizebox{#2}{#3}{\includegraphics[#6draft=true,type=\pdfpicFileType,ext=.\pdfpicFileExt,read=*,command=##1]{#4}}}%
\else%
%%
%% Normal picture: image in the specified format.
\resizebox{#2}{#3}{\includegraphics[#6type=\pdfpicFileType,ext=.\pdfpicFileExt,read=*,command=##1]{#4}}\fi}\fi%
}

%% Simpler version to keep LaTeX2HTML from getting confused
\begin{imagesonly}
\renewcommand{\pspic}[4][\psall]{\resizebox{#2}{#3}{\includegraphics{ps/#4.ps}}}
\end{imagesonly}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%>> To do (6/2002): 
%% It would be nice to have some sort of facility for automatically 
%% handling conditional text for different document types.  Here's
%% a sketch, but it is not legal LaTeX code:
%%
%% \newcommand{\definedocumenttype}[2]{
%%   \expandafter\def\csname dt#1\endcsname{#2}%
%%   \newcommand{not#1}[1]{}%
%%   \newcommand{#1only}[1]{}%
%% }
%% \definedocumenttype{book}{100}          % Book
%% \definedocumenttype{thesis}{80}         % PhD. or Master's thesis
%% \definedocumenttype{techreport}{60}     % Technical report
%% \definedocumenttype{preprint}{45}       % Journal preprint (to be passed around, not submitted)
%% \definedocumenttype{journal}{40}        % Journal paper (as published, or to be submitted)
%% \definedocumenttype{conf}{20}           % Conference paper
%% \definedocumenttype{article}{0}         % Default; generic article
%% 
%% \newcount\documenttype \documenttype=0
%% \newcommand{\setdocumenttype}[1]{%
%%   \documenttype=#1%
%%   \newcommand{not#1}[1]{#1}%
%%   \newcommand{#1only}[1]{}%
%% }
%%
%% Usage:
%%  \setdocumenttype{\book}  % Or any other
%%  \bookonly{Text for the book version}
%%  \notbook{Text for all versions except the book}
%%
%% All 'only' and 'not' comparisons should be available
%% even if only a single document type is available.  It should
%% be legal to define multiple document types.  However, it's not
%% clear how to implement any of this.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  Standard lengths, used to keep documents uniform throughout
 
%% Set size of windowpane to fit one, two, etc. square panes per line  
%%
\newlength{\oneplotwidth}           \setlength{\oneplotwidth}         {\textwidth}
\newlength{\twoplotwidth}           \setlength{\twoplotwidth}         {0.46\textwidth}
\newlength{\twoplotheight}          \setlength{\twoplotheight}        {\twoplotwidth}
\newlength{\threeplotwidth}         \setlength{\threeplotwidth}       {0.31\textwidth}
\newlength{\threeplotheight}        \setlength{\threeplotheight}      {\threeplotwidth}
\newlength{\fourplotwidth}          \setlength{\fourplotwidth}        {0.22\textwidth}
\newlength{\fourplotheight}         \setlength{\fourplotheight}       {\fourplotwidth}
\newlength{\fiveplotwidth}          \setlength{\fiveplotwidth}        {0.18\textwidth}
\newlength{\fiveplotheight}         \setlength{\fiveplotheight}       {\fiveplotwidth}
 
%% Set size of windowpane to fit the specified configuration of square
%% panes per page  
%%
\newlength{\twobytwoplotwidth}      \setlength{\twobytwoplotwidth}    {0.46\textwidth}
\newlength{\threebyfourplotwidth}   \setlength{\threebyfourplotwidth} {0.25\textwidth}
\newlength{\fourbythreeplotwidth}   \setlength{\fourbythreeplotwidth} {0.171875\textheight}
%% Note that the portrait page above with 12 square panes is named as 
%% a "width", but it is actually limited in the vertical direction
%% for typical US paper proportions, assuming there is a 1-inch caption.
 
 
%% Plot width that xmgr graphs should use
%%
%% This value is appropriate for output that has been run through
%% ps2epsi to fix the bounding boxes.  Xmgr computes them too
%% generously, so this would need to be some smaller value otherwise.
%%
\newlength{\xmgrplotwidth}          \setlength{\xmgrplotwidth}{\textwidth}
 
 
%% Blank variable available for various purposes
%%   Must use \setlength or \settowidth to give it 
%%   a value before using it
%%   E.g.: \settowidth{\templength}{Some text}
%%
\newlength{\templength}

 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Support for captioned subfigures
%%
%% To enable these commands, add "\usepackage[tight,center]{subfigure}"
%% before loading this file.  Then define subfigures with \sfobject, \sfpic,
%% or \sfpicframe, and refer to them with \sfref or \sfrefnp.
%%
%% Requires subfigure package version 2.1.2 or higher.  See the subfigure 
%% documentation for more details, such as how to change the caption 
%% separation, fonts, etc.:
%% http://www-2.cs.cmu.edu/afs/cs/usr/sdc/www/latex/subfigure.html
%%
\makeatletter
  \@ifpackageloaded{subfigure}{%

  %% Set up the subfigure package to italicize only the subfigure letters,
  %% not the parentheses, and to make \ref show only the bare letters,
  %% without any parentheses and without the main figure number.
  \let\p@subfigure\relax
  \renewcommand{\thesubfigure}{\emph{\alph{subfigure}}}
  \renewcommand*{\@thesubfigure}{(\thesubfigure)\hskip\subfiglabelskip}
  \renewcommand*{\@@thesubfigure}{(\thesubfigure)}


  %% Define a subfigure of any type with a caption underneath it
  %% Usage:   \sfobject[width]{item}{caption-text}{subfigure-label}
  %% Example: \sfobject{0.3\textwidth}{... a picture of some sort ...}{Above is a fancy picture}{fig}
  %% The subfigure-label must be unique for the whole document.
  %%
  \newcommand{\sfobject}[4]{%
    \subfigure[\label{sf:#4}#3]{\begin{minipage}[t]{#1}#2\end{minipage}}}
  \newcommand{\sfobjectuncaptioned}[2]{% Same spacing but no caption
    \subfigure{\begin{minipage}[t]{#1}#2\end{minipage}\addtocounter{subfigure}{-1}}}


  %% Define a subfigure consisting of a captioned \pdfpic
  %% Usage:   \sfpic{width}{filenamebase}{imagetype}{caption text}{subfigure-label}
  %% Example: \sfpic{0.3\textwidth}{picture}{jpg}{A picture}{renoir-pic}
  %%
  \newcommand{\sfpic}[5]{%
    \sfobject{#1}{\pdfpic{\textwidth}{!}{#2}{#3}}{#4}{#5}}%
  \newcommand{\sfpicuncaptioned}[3]{% Same but no caption
    \sfobjectuncaptioned{#1}{\pdfpic{\textwidth}{!}{#2}{#3}}}%

  %% Same as \sfpic but with a frame around the picture
  \newcommand{\sfpicframe}[5]{%
    \sfobject{#1}{\frame{\pdfpic{\textwidth}{!}{#2}{#3}}}{#4}{#5}}%
  \newcommand{\sfpicframeuncaptioned}[3]{%
    \sfobjectuncaptioned{#1}{\frame{\pdfpic{\textwidth}{!}{#2}{#3}}}}%


  %% Expand a reference to a subfigure, e.g. in caption or the main text
  %% \sfref{subfigure-label} yields (\emph{a}), etc.
  \newcommand{\sfref}[1]{(\ref{sf:#1})}


  %% Same as \sfref without the parentheses
  %% \sfrefnp{subfigure-label} yields \emph{a}, etc.
  \newcommand{\sfrefnp}[1]{\ref{sf:#1}}


  %% If producing overhead slides, call this command in the preamble
  %% so that (a), (b), etc. will be omitted from subfigure captions
  \newcommand{\sfstriplabels}{\renewcommand*{\@thesubfigure}{\mbox{}}}
}
\makeatother



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  Misc

%% Puts a tiny note in the margin; useful for notes on drafts.
%%
%% To disable all of them uncomment the second def.
%% When you use it in the middle of a paragraph, you should follow 
%% the last brace with a comment character (%) to avoid getting
%% a double space in the output.
\newcommand{\draftnote}[1]{{\marginpar{\tiny\em\raggedright #1}}}
%%\renewcommand{\draftnote}[1]{}

%% The \draftnote command is based on \marginpar, which doesn't work 
%% in floating  bodies like figures and tables because the notes also
%% float.  So we provide a non-floating version of marginpar
%% (\rawmarginpar), and then use that to create a version of
%% \draftnote that works with figures (\rawdraftnote).  Note that
%% \rawdraftnotes might overlap, go off the page, etc.; they are not
%% juggled automatically like \draftnotes are.  \rawdraftnote
%% usually works best right before the figure caption.
%%
\newcommand{\rawmarginpar}[1]{%
\vadjust{\smash{\llap{\parbox[t]{0.7\marginparwidth}{#1}\kern\marginparsep}}}}
\newcommand{\rawdraftnote}[1]{{\rawmarginpar{\tiny\em\raggedright #1}}}

%% Pretends that its argument takes zero horizontal space, e.g. to 
%% prevent a caption from having a linebreak by letting it 
%% extend slightly into the space on either side.
%%
\providecommand{\zerospace}[1]{\mbox{\makebox[0in]{#1}}}

%% Same as \zerospace except that the result is left-
%% justified, as if it had zero length out to the right.
\providecommand{\zerolength}[1]{\mbox{\makebox[0in][l]{#1}}}


%% Centers the given object vertically and horizontally
%% within a square box of the specified size, ignoring 
%% the size of the object.  
%%
%% Usage: \squarebox[position]{width}{object}
%%
%% Examples:
%%   Center some text in the left 1/10 page and draw a border around it:
%%     \frame{\squarebox{0.1\textwidth}{Some text}}
%%   Center an image 1/8 the size of the page in a box twice its width:
%%     \frame{\squarebox{0.25\textwidth}{\pdfpic{0.5\textwidth}{!}{somefile}{pdf}}
\newcommand{\squarebox}[3][c]{%
    \begin{minipage}[#1]{#2}%
      \setlength{\unitlength}{\textwidth}%
      \begin{picture}(1.0,1.0)%
        \put(0.5,0.5){\makebox(0,0)[c]{#3}}%
      \end{picture}%
    \end{minipage}}

%% Command to add a degree symbol following a number
%%
%% When using it, you need to follow it with a "\ " if the next
%% character should be a space.  
%%
%% Examples: "23\degree\ line"    "the orientation was 23\degree."
%%
%% Used to be called \deg but there is now a LaTeX2e command by that
%% name. 
\newcommand{\degree}{\ensuremath{^\circ}}


%% Non-math-mode equivalents of math-mode characters, etc.
%% These are useful for preventing LaTeX2HTML from converting
%% tiny in-text expressions like these into GIFs, and can also 
%% make text a little more readable overall.
\newcommand{\superscript}[1]{\ensuremath{^#1}}
\newcommand{\subscript}[1]{\ensuremath{_#1}}
\newcommand{\mtimes}[2]{\ensuremath{#1 \times #2}}
\newcommand{\madd}[2]{\ensuremath{#1 + #2}}
\newcommand{\mplus}{\ensuremath{+}}
\newcommand{\mpm}{\ensuremath{\pm}}
\newcommand{\mlt}{\ensuremath{<}}
\newcommand{\mgt}{\ensuremath{>}}

%% Given a color type as argument, e.g. \psmono or \pscolor, returns the note 
%% that should be placed in the caption for that figure.
%% This will make figures that require color say so; I can't think of anything
%% useful for the rest to say.
%% Maybe \pscolororbw should say something like "(Figure looks better in color)"?
\newcommand{\figurenote}[1]{%
\ifx#1\pscolor{\ ({\em color figure\/})}\fi}


%% Dummy command marking a section of text as something for latex2html
%% to typeset as a single left-justified block  
\newcommand{\htmlblock}[1]{#1}


%% Constructs a titled figure caption.  Takes four arguments:
%%
%% \titledcaption[category]{label}{title}{captiontext}
%%
%% The "category" argument is optional; if present it should indicate the
%% type of image the file represents, i.e.  \psline for a line drawing,
%% \pscolor for a color photo, \pscolororbw for an image that is readable
%% either in color or monochrome, \psnone for a blank space, etc.  At
%% present, "category" is only used to see whether or not to
%% add a descriptive note for the title and list of figures entry.
%% See the \figurenote command for the cases where a note will be
%% added.  The default will never add any note.
%% 
%% The "label" is a name used to construct a label for the figure.
%%
%% The "title" should be a short heading, which will go in bold at the
%% top of the caption, and also goes into the list of figures.
%%
%% The "captiontext" will go into the caption only, not the list of
%% figures, after the title.  Just use an empty last argument {} if 
%% there is no caption text.
%% 
%% Complete figure example:
%% \begin{figure}
%%   \centering 
%%   \pspic[\psline]{\oneplotwidth}{!}{some-figure-filename-wo-ps-extension}
%%   \titledcaption[\psline]{fg:some-figure-label}
%%   {Title of the figure}{ 
%%     Some long text describing what this figure means and how it
%%     should be interpreted.}
%% \end{figure}
%%
%% jbednar040510: For some reason, I had replaced both "#1"s with 
%% "\protect{#1}", probably to fix some problem with the separate
%% versions for typesetters (below).  However, that broke the color
%% figure labels for the normal case, so I have removed it.  Next time
%% the typesetter versions are used, they will probably need to be
%% debugged.
%%
\newcommand{\titledcaption}[4][\psall]{%
    \caption[#3\figurenote{#1}]{%
      \label{#2}\mycapdefs%
      \textbf{\mathversion{bold}#3\figurenote{#1}.} %
      \htmlblock{#4}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Support for defining figure graphics separately from captions
%%
%% To use this, just pick a label you want to refer to the figure by,
%% and define the meat of the figure:
%%
%% \definefigbody{fg:some-fig}{%
%%  \sfpicframe{\twoplotwidth}{picture1}{jpg}{Case 1}{case-1-label}\hfill
%%  \sfpicframe{\twoplotwidth}{picture2}{jpg}{Case 2}{case-2-label}}
%%
%% Then wherever you want the figure to appear, insert it with a caption:
%%
%%  \insertfig[\pscolor]{fg:some-fig}{%
%%    Figure title}{%
%%    This figure conclusively demonstrates that...}%
%%
%% Leave off [\pscolor] if you don't want the "(color figure)" note
%% in the caption.
%%
%% Everything else will be handled automatically.  If you want fine
%% control over the figure (instead of automatically using
%% titledcaption, fullfigure*, etc.), just use 
%% \insertfigbody{fg:some-fig} to insert the meat of the figure into 
%% your own figure skeleton.
%%
%% If you also want to define the captions separately from where they
%% are first inserted into the text, then use \definefigcaption
%% instead of \insertfig.  That way the caption will be defined but
%% not yet inserted into the text.  Then just use \firstfigref
%% instead of \ref the first time you refer to the figure, and the
%% figure will automatically be placed into the text at that point.
%%
%% If you want the captioned figure to be placed somewhere other
%% than the first reference, just put an \insertfighere{fg-some-fig} 
%% command where you want the figure to appear.
%%
%%
%% Defines the body of the given figure
\newcommand{\definefigbody}[2]{%
  \ifundefined{figbody--#1}\expandafter\def\csname figbody--#1\endcsname{#2}%
  \else\errmessage{Figure #1 already defined}\fi}%
%%
%% Rarely used by end users:
\newcommand{\insertfigbody}[1]{\csname figbody--#1\endcsname}%
\newcommand{\insertfigtype}[1]{\csname figtype--#1\endcsname}%
\newcommand{\insertfigtitle}[1]{\csname figtitle--#1\endcsname}%
\newcommand{\insertfigcaption}[1]{\csname figcaption--#1\endcsname}%
%%
%% Defines the type, title, and caption of the given figure
\newcommand{\definefigcaption}[4][\psmono]{%
  \ifundefined{figtype--#2}\expandafter\def\csname figtype--#2\endcsname{#1}%
  \else\errmessage{Type for #2 already defined}\fi%
  \ifundefined{figtitle--#2}\expandafter\def\csname figtitle--#2\endcsname{#3}%
  \else\errmessage{Title for #2 already defined}\fi%
  \ifundefined{figcaption--#2}\expandafter\def\csname figcaption--#2\endcsname{#4}%
  \else\errmessage{Caption for #2 already defined}\fi}%
%%
%% Inserts the given figure given the type, title, and caption
\newcommand{\insertfig}[4][\psmono]{%
  \begin{fullfigure*}\insertfigbody{#2}\titledcaption[#1]{#2}{#3}{#4}\end{fullfigure*}}%
%%
%% Rarely used by end users:
\newcommand{\insertfighere}[1]{%
  \insertfig%
  [\insertfigtype{#1}]{#1}%
  {\insertfigtitle{#1}}%
  {\insertfigcaption{#1}}}%
%%
%% Refers to and inserts the given captioned figure
\newcommand{\firstfigref}[1]{\ref{#1}\insertfighere{#1}}%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Support for figures at end of document for journal paper
%% submissions
%% 
%% None of these commands are used in a normal camera-ready paper
%%
%% For these commands to work, you should use \firstfigref
%% consistently (which allows the actual caption to be inserted 
%% wherever).  
%%
%% If you use subfigures, you should also add a line:
%%   \PassOptionsToPackage{normalsize}{subfigure}
%% before the \usebpackage{subfigure}, to make the fonts the right 
%% size.


%% Declare that figures should be put at end of paper for typesetting
\newcommand{\figuresatend}[1]{%
  \renewcommand{\firstfigref}[1]{\begin{center}--- Insert
      figure~\ref{##1} about here ---\end{center}\ref{##1}}%
  %% Hack to make subfigure package work outside of a float environment
  \makeatletter\newcommand{\@captype}{figure}\makeatother%
}

%% Override this if you need to add your name or manuscript number
%% Accepts one argument, the figure key (suitable for \ref)
\newcommand{\submissionfigdescription}[1]{Figure~\ref{#1}}

% Format a figure for typesetting
% Usage: \insertsubmissionfig[separation]{reference}
\newcommand{\insertsubmissionfig}[2][1in]{%
\newpage\setcounter{subfigure}{0}
\centering
\makebox[0in]{%
\resizebox{7.5in}{!}
{\begin{minipage}{\textwidth}
    \centering%
    \insertfigbody{#2}\\[#1]
    \submissionfigdescription{#2}
  \end{minipage}}}%
}


% Format a caption for typesetting
% Usage: \insertsubmissioncaption{reference}
\newcommand{\insertsubmissioncaption}[1]{%
  \newpage%
  \begin{figure}[h]%
    \renewcommand{\baselinestretch}{1.5}\small\normalsize
    \caption[\insertfigtitle{#1}\figurenote{\protect{\insertfigtype{#1}}}]{%
      \label{#1}%
      \textbf{\insertfigtitle{#1}\figurenote{\protect{\insertfigtype{#1}}}}.
      \raggedright%
      \htmlblock{\insertfigcaption{#1}}}
  \end{figure}%
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Tech report title pages
%%
%% Default values; you can (and should) override these using
%% \renewcommand within your own paper.  Often you will need to add
%% different linebreaks to the \techreporttitle and
%% \techreportauthor since they need to fit in such a narrow window.
%%
\newcommand{\techreporttitle}{\title}
\newcommand{\techreportauthor}{\author}
\newcommand{\techreportnumber}{}
\newcommand{\techreportemailaddress}{}
\newcommand{\techreporthttpaddress}{http://www.cs.utexas.edu/users/nn}
\newcommand{\techreportdepartment}{Artificial Intelligence Laboratory}
\newcommand{\universityname}{The University of Texas at Austin}
\newcommand{\universityaddress}{Austin, TX 78712}

%% Call just after your \begin{document} to actually generate the tech
%% report title page.
%%
%% Takes two arguments -- the offset in x and y to correct for the
%% left and top margins, respectively, in the current style.  The
%% values should both be zero for the default 1-inch margins in
%% nnonecolumn.sty; adjust other margins as needed.
%%
\newcommand{\techreporttitlepage}[2]{%
  \newpage
  \thispagestyle{empty}
  \setlength{\unitlength}{1in}%
  \begin{picture}(0,0)(#1,#2)
    \put(1,-2.3){\parbox{4in}{%
      \begin{center}%
        {\textbf{\Large \techreporttitle}}\\[8mm]
        {\textbf{\large \techreportauthor}}\\[8mm]
        \textbf{\large \techreportnumber}
      \end{center}}}
    \put(1,-7.8){\parbox{4in}{%
      \begin{center}%
        {\tt \techreportemailaddress}\\
        {\tt \techreporthttpaddress}\\[8mm]
        \techreportdepartment\\
        \universityname\\
        \universityaddress
      \end{center}}}
  \end{picture}
  \newpage
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% For emacs:
%Local Variables:
%TeX-command-default:"Check"
%End:

